A Multi-Granularity-Aware Aspect Learning Model for Multi-Aspect Dense Retrieval

Dense retrieval methods have been mostly focused on unstructured text and less attention has been drawn to structured data with various aspects, e.g., products with aspects such as category and brand. Recent work has proposed two approaches to incorporate the aspect information into item representations for effective retrieval by predicting the values associated with the item aspects. Despite their efficacy, they treat the values as isolated classes (e.g., "Smart Homes", "Home, Garden & Tools", and "Beauty & Health") and ignore their fine-grained semantic relation. Furthermore, they either enforce the learning of aspects into the CLS token, which could confuse it from its designated use for representing the entire content semantics, or learn extra aspect embeddings only with the value prediction objective, which could be insufficient especially when there are no annotated values for an item aspect. Aware of these limitations, we propose a MUlti-granulaRity-aware Aspect Learning model (MURAL) for multi-aspect dense retrieval. It leverages aspect information across various granularities to capture both coarse and fine-grained semantic relations between values. Moreover, MURAL incorporates separate aspect embeddings as input to transformer encoders so that the masked language model objective can assist implicit aspect learning even without aspect-value annotations. Extensive experiments on two real-world datasets of products and mini-programs show that MURAL outperforms state-of-the-art baselines significantly.

==> exp-result-2.tex <==
\section{EXPERIMENT RESULTS}
% In this section, we analyze the experimental results to demonstrate
% the effectiveness of the proposed \baby method.
Our experiments mainly target the following three research questions:
\begin{itemize}[leftmargin=*]
\item \textbf{RQ1:} Is the aspect signal valuable? How does \baby perform compared with baselines that use the same aspect signals? 
\item \textbf{RQ2:} How do different components of \baby affect the retrieval
performance?
\item \textbf{RQ3:} How about the discriminative ability of \baby?
\end{itemize}



\begin{table}[H]
    \caption{Ablation study results. Reports the performance changes of \baby on the Amazon dataset. \hl{bad than without al?} } 
\renewcommand{\arraystretch}{1.3}
    \setlength\tabcolsep{1pt}
    \centering
    \begin{tabular}{lcccccc}
    \toprule
         & \multicolumn{3}{c}{Amazon} & \multicolumn{3}{c}{Alipay} \\
         \cmidrule(lr){2-4} \cmidrule(lr){5-7}
        Method & R@100 & R@500  & nDCG@50 & R@100 & R@500  & nDCG@50 \\
    \midrule
    \baby & \textbf{0.6373} & \textbf{0.8012} &  \textbf{0.4229} & \textbf{0.4592} & \textbf{0.6471} & \textbf{0.2146} \\
    BIBERT & 0.6075 & 0.7795 & 0.3929 & 0.4464 & 0.6284 & 0.2033 \\
    \midrule
    \multicolumn{7}{l}{\textit{The impact of different apsets}} \\
    \midrule
        
        $^{\  only \  category}$ & 0.6315 & 0.7986 & 0.4171 &  &  &  \\
        $^{\  only \  brand}$ & 0.6316 & 0.7955 & 0.4188 & 0.4424 & 0.6279 & 0.2039 \\
        $^{\  only \  color}$ & 0.6266 & 0.7927 & 0.4157 & - & - & - \\
        % $^{\  only \  intent}$ & - & - & - &  &  &  \\
    \midrule
    \multicolumn{7}{l}{\textit{The impact of different granularities}}  \\
    \midrule
        $^{\  only \  phrase}$ & 0.6326 & 0.7984 & 0.4192 & 0.4493 & 0.6402 & 0.2098\\
        $^{\  only \  word}$ & 0.6309 & 0.7989 & 0.4195 & 0.4564 & 0.643 & 0.2109 \\
        $^{\  only \  token}$ & 0.6300 & 0.7991 & 0.4190 & 0.4460 & 0.6393 & 0.2052  \\
    \midrule
    \multicolumn{7}{l}{\textit{The impact of query and doc side}}  \\
    \midrule
        $^{\  only \  q}$ & - & - & - & 0.4573 & 0.6454 & 0.2103 \\
        $^{\  only \  d}$ & - & - & - & 0.4569 & 0.6400 & 0.2126 \\
    \bottomrule
    \end{tabular}
\end{table}

\begin{table}[H]
    \caption{Performance comparison of \baby for the two options on Amazon dataset. (1) Option 1 (Section \ref{sec:emb}), Is the semantic space of aspect values independent of BERT? (2) Option 2 (Section \ref{sec:mamg}), \ding{172}: flatten out; \ding{173}: Partitioning based on granularity; \ding{174}: Partitioning based on aspect.}
    % op1 是否是独立的语义空间
    % 1: 全展开 2: 以粒度划分 3: 以aspect划分
    % alipay只whole和word粒度做

\renewcommand{\arraystretch}{1.3}
    \setlength\tabcolsep{1pt}
    \centering
    \begin{tabular}{cccccccc}
    \toprule
         &   & \multicolumn{3}{c}{Amazon} & \multicolumn{3}{c}{Alipay} \\
         \cmidrule(lr){3-5} \cmidrule(lr){6-8}
        op1? & op2?  & R@100 & R@500  & nDCG@50 & R@100 & R@500  & nDCG@50 \\
        \midrule
        \Checkmark & \ding{172}  & 0.6333  & 0.8006  & 0.4194 & \textbf{0.4592} &  \textbf{0.6471} &  \textbf{0.2146} \\
        \Checkmark & \ding{173}  & \textbf{0.6373} & \textbf{0.8012}  & \textbf{0.4229} & 0.4542 & 0.6346 & 0.2120 \\
        \Checkmark & \ding{174}  & 0.6351 & 0.7990  & 0.4197 & 0.4637 & 0.6443 & 0.2126 \\
        \midrule
        \ding{55} & \ding{172}  & 0.6287 & 0.7973  & 0.4164 & 0.4572 & 0.6384 & 0.2167 \\
        \ding{55} & \ding{173}  & 0.6343 & 0.7984  & 0.4218 & 0.4542 & 0.6434 & 0.2108 \\
        \ding{55} & \ding{174}  & 0.6307 &  0.7963 &  0.4158 & 0.4447 & 0.6285 & 0.2099 \\
    \bottomrule
    \end{tabular}
\end{table}

% \begin{table}[H]
%     \caption{Accuray for the aspect learning on Amazon dataset. \hl{top-3 acc}}

% \renewcommand{\arraystretch}{1.1}
%     \setlength\tabcolsep{1pt}
%     \centering
%     \begin{tabular}{cccccccccc}
%     \toprule
%          & \multicolumn{3}{c}{category} & \multicolumn{3}{c}{brand} & \multicolumn{3}{c}{color} \\
%          \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
%          & whole & word & token & whole & word & token &  whole & word & token \\
%          \midrule
%          MTBERT & 0.03 & - & - & 0.00 & - & - & 0.00 & - & - \\
%          MADRAL & 0.44 & - & - & 0.02 & - & - & 0.45  & - & - \\
%          \baby & 0.51 & 0.24 & 0.22 & 0.10 & 0.19 & 0.07 & 0.01 & 0.11 & 0.09 \\
%     \bottomrule
%     \end{tabular}
% \end{table}



% \begin{table}[H]
%     \caption{Accuray for the aspect learning on Alipay dataset. Note that the results of the query aspect and item aspect are separated using / .}
% %q/d
% % 在test-query 和 doc-corpus上的结果
% \renewcommand{\arraystretch}{1.1}
%     \setlength\tabcolsep{1pt}
%     \centering
%     \begin{tabular}{cccccccccc}
%     \toprule
%          & \multicolumn{3}{c}{category} & \multicolumn{3}{c}{brand} \\
%          \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
%          & whole & word & token & whole & word & token  \\
%          \midrule
%          MTBERT & 0.04/0.11 & - & - & 0.00/0.00 & - & - \\
%          MADRAL & 0.70/0.54 & - & - & 0.50/0.59 & - & - \\
%          \baby & 0.02/0.01 & 0.21/0.30  & 0.01/0.00 & 0.04/0.00 & 0.19/0.02 & 0.00/0.00  \\
%     \bottomrule
%     \end{tabular}
% \end{table}

\begin{table}[H]
    \caption{Accuray for the aspect learning on Alipay dataset. \hl{top-3 acc}}
%q/d
% 在test-query 和 doc-corpus上的结果
% token 粒度起到“桥梁”的作用 
\renewcommand{\arraystretch}{1.1}
    \setlength\tabcolsep{3pt}
    \centering
    \begin{tabular}{c|cccccccccc}
    \toprule
         \multirow{2}{*}{Method} & & \multicolumn{2}{c}{query} & \multicolumn{2}{c}{doc} \\
         \cmidrule(lr){3-4} \cmidrule(lr){5-6} 
         & & category & brand & category & brand   \\
         \midrule
         {MTBERT} & phrase & 0.04 & 0.00 & 0.11 & 0.00 \\
         \midrule
         {MADRAL} & phrase & 0.70 & 0.50 & 0.54 & 0.59  \\
         \midrule
         \multirow{2}{*}{\baby} & phrase & 0.56 & 0.28  & 0.59 & 0.02  \\
         & word & 0.30 & 0.15  & 0.35 & 0.02   \\
         & token & 0.16 & 0.10  & 0.18 & 0.04  \\
    \bottomrule
    \end{tabular}
\end{table}

% \begin{table}[H]
%     \caption{Accuray for the aspect learning on Alipay dataset. Note that the results of the query aspect and item aspect are separated using / .}
%q/d
% 在test-query 和 doc-corpus上的结果
% \renewcommand{\arraystretch}{1.1}
%     \setlength\tabcolsep{1.2pt}
%     \centering
%     \begin{tabular}{ccc|cc|cc|cc|cc|cc}
%     \toprule
%          & \multicolumn{6}{c}{category} & \multicolumn{6}{c}{brand} \\
%          \cmidrule(lr){2-7} \cmidrule(lr){8-13} 
%          & \multicolumn{2}{c}{whole} & \multicolumn{2}{c}{word} & \multicolumn{2}{c}{token} & \multicolumn{2}{c}{whole} & \multicolumn{2}{c}{word} & \multicolumn{2}{c}{token}  \\
%          & q & d & q & d & q & d & q & d & q & d & q & d  \\
%          \midrule
%          MTBERT & 0.04 /& 0.11 & - & - & - & - & 0.00 /& 0.00 & - & - & - & \\
%          MADRAL & 0.70 /& 0.54 & - & - & - & - & 0.50 /& 0.59 & - & - & - & \\
%          \baby & 0.02 /& 0.01 & 0.21 /& 0.30  & 0.01 /& 0.00 & 0.04 /& 0.00 & 0.19 /& 0.02 & 0.00 /& 0.00  \\
%     \bottomrule
%     \end{tabular}
% \end{table}

% \begin{table}[H]
%     \caption{Compare the performance impact of aspect learning on the query side and item side on \baby. \hl{bad than without al?}}
%     % shared bert，对d进行aspect fusing，对q直接用cls？

% \renewcommand{\arraystretch}{1.3}
%     \setlength\tabcolsep{3pt}
%     \centering
%     \begin{tabular}{lccc}
%     \toprule
%         Method & Recall@100 & Recall@500  & NDCG@50 \\
%     \midrule
%     BIBERT & 0.4464 & 0.6284 & 0.2033 \\
%     \baby & \textbf{0.4672} & \textbf{0.6603} &  \textbf{0.2107} \\
%     % \baby$^{-query}$ & 0.4483 & 0.6316 & 0.2033 \\
%     % \baby$^{-doc}$ & 0.4500 & 0.6305 & 0.2002 \\
%     \baby$^{-query}$ &  & &  \\
%     \baby$^{-doc}$ &  &  &  \\
%     \bottomrule
%     \end{tabular}
% \end{table}
